Benchmarking Robustness of AI-Enabled Multi-sensor Fusion Systems: Challenges and Opportunities

Multi-Sensor Fusion (MSF) based perception systems have been the foundation in supporting many industrial applications and domains, such as self-driving cars, robotic arms, and unmanned aerial vehicles. Over the past few years, the fast progress in data-driven artificial intelligence (AI) has brought a fast-increasing trend to empower MSF systems by deep learning techniques to further improve performance, especially on intelligent systems and their perception systems. Although quite a few AI-enabled MSF perception systems and techniques have been proposed, up to the present, limited benchmarks that focus on MSF perception are publicly available. Given that many intelligent systems such as self-driving cars are operated in safety-critical contexts where perception systems play an important role, there comes an urgent need for a more in-depth understanding of the performance and reliability of these MSF systems. To bridge this gap, we initiate an early step in this direction and construct a public benchmark of AI-enabled MSF-based perception systems including three commonly adopted tasks (i.e., object detection, object tracking, and depth completion). Based on this, to comprehensively understand MSF systems' robustness and reliability, we design 14 common and realistic corruption patterns to synthesize large-scale corrupted datasets. We further perform a systematic evaluation of these systems through our large-scale evaluation. Our results reveal the vulnerability of the current AI-enabled MSF perception systems, calling for researchers and practitioners to take robustness and reliability into account when designing AI-enabled MSF.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> tab/benchCorruption.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[]
% \label{tab: corruption}
% \resizebox{0.95\linewidth}{!}{%

% \begin{tabular}{llll}
% \textbf{Category}                                                                                      & \textbf{Corruptiom} & \textbf{Potential Reasons}                                                                                                                                                     & \textbf{Modal} \\
% \rowcolor[HTML]{BFBFBF} 
% \cellcolor[HTML]{BFBFBF}                                                                               & Rain (RN)           & \cellcolor[HTML]{BFBFBF}                                                                                                                                                       & C,L            \\
% \rowcolor[HTML]{BFBFBF} 
% \cellcolor[HTML]{BFBFBF}                                                                               & Fog (FG)            & \cellcolor[HTML]{BFBFBF}                                                                                                                                                       & C,L            \\
% \rowcolor[HTML]{BFBFBF} 
% \cellcolor[HTML]{BFBFBF}                                                                               & Brightness (BR)     & \cellcolor[HTML]{BFBFBF}                                                                                                                                                       & C              \\
% \rowcolor[HTML]{BFBFBF} 
% \multirow{-4}{*}{\cellcolor[HTML]{BFBFBF}\begin{tabular}[c]{@{}l@{}}Weather\\ Corruption\end{tabular}} & Darkness (DK)       & \multirow{-4}{*}{\cellcolor[HTML]{BFBFBF}\begin{tabular}[c]{@{}l@{}}natural weather~\cite{},\\ lightning conditions\\ change~\cite{};\end{tabular}}                            & C              \\
%                                                                                                        & Distortion (DT)     &                                                                                                                                                                                & C              \\
%                                                                                                        & Motion Blur (MB)    &                                                                                                                                                                                & C              \\
% \multirow{-3}{*}{\begin{tabular}[c]{@{}l@{}}Sensor \\ Corruption\end{tabular}}                         & Defocus Blur (DB)   & \multirow{-3}{*}{\begin{tabular}[c]{@{}l@{}}lens distortion~\cite{},\\ moves quickly~\cite{}\\ loses focus~\cite{},\end{tabular}}                                              & C              \\
% \rowcolor[HTML]{BFBFBF} 
% \cellcolor[HTML]{BFBFBF}                                                                               & Image Gaussion (GN) & \cellcolor[HTML]{BFBFBF}                                                                                                                                                       & C              \\
% \rowcolor[HTML]{BFBFBF} 
% \cellcolor[HTML]{BFBFBF}                                                                               & Point Gaussion (GN) & \cellcolor[HTML]{BFBFBF}                                                                                                                                                       & L              \\
% \rowcolor[HTML]{BFBFBF} 
% \cellcolor[HTML]{BFBFBF}                                                                               & Image Impulse (IN)  & \cellcolor[HTML]{BFBFBF}                                                                                                                                                       & C              \\
% \rowcolor[HTML]{BFBFBF} 
% \multirow{-4}{*}{\cellcolor[HTML]{BFBFBF}\begin{tabular}[c]{@{}l@{}}Noise\\ Corruption\end{tabular}}   & Point Impulse (IN)  & \multirow{-4}{*}{\cellcolor[HTML]{BFBFBF}\begin{tabular}[c]{@{}l@{}}low ranging accuracy~\cite{},\\ mechanical vibration~\cite{},\\ strong illumination~\cite{};\end{tabular}} & L              \\
%                                                                                                        & Spatial (SM)        &                                                                                                                                                                                & A              \\
% \multirow{-2}{*}{\begin{tabular}[c]{@{}l@{}}Sensor \\ Misalignment\end{tabular}}                       & Temporal (TM)       & \multirow{-2}{*}{\begin{tabular}[c]{@{}l@{}}mechanical vibrations~\cite{},\\ transmission delay~\cite{};\end{tabular}}                                                         & A             
% \end{tabular}


% }
% \end{table}



\begin{table}[t]
\caption{Corruption patterns used in this study.}
\vspace{-10pt}
\label{tab: corruption}
\centering
\resizebox{0.95\linewidth}{!}{%
\scriptsize
\begin{tabular}{llc}
\toprule
\textbf{Category}                                                              & \textbf{Corruption}             & \textbf{Modality} \\
\midrule
                                                                                                       & Rain (RN)                       & Camera \& LiDAR            \\
                                                                                                       & Fog (FG)                        & Camera \& LiDAR            \\
                                                                                                       & Brightness (BR)                 & Camera              \\
\multirow{-4}{*}{\begin{tabular}[c]{@{}l@{}}Weather\\ Corruption\end{tabular}}                         & Darkness (DK)                   & Camera              \\
\rowcolor{lightgray} 
\cellcolor{lightgray}                                                                               & Distortion (DT)                 & Camera              \\
\rowcolor{lightgray} 
\cellcolor{lightgray}                                                                               & Motion Blur (MB)                & Camera              \\
\rowcolor{lightgray} 
\cellcolor{lightgray}                                                                               & Defocus Blur (DB)               & Camera              \\
\rowcolor{lightgray} 
\cellcolor{lightgray}                                                                               & Image Gaussian Noise (GN)       & Camera              \\
\rowcolor{lightgray} 
\cellcolor{lightgray}                                                                               & Point Cloud Gaussian Noise (GN) & LiDAR              \\
\rowcolor{lightgray} 
\cellcolor{lightgray}                                                                               & Image Impulse Noise (IN)        & Camera              \\
\rowcolor{lightgray} 
\multirow{-7}{*}{\cellcolor{lightgray}\begin{tabular}[c]{@{}l@{}}Sensor \\ Corruption\end{tabular}} & Point Cloud Impulse Noise (IN)  & LiDAR              \\
                                                                                                       & Spatial Misalignment (SM)       &  Camera \& LiDAR             \\
\multirow{-2}{*}{\begin{tabular}[c]{@{}l@{}}Sensor \\ Misalignment\end{tabular}}                       & Temporal Misalignment (TM)      &          Camera \& LiDAR    
\\\bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{table}





% ori table
% \begin{table}[t]
% \caption{Corruption patterns used in this study. C and L represent camera and LiDAR, A represents sensor-misalignment, respectively.\wang{update this table.}}
% \label{tab: corruption}
% \centering
% \small
% \begin{tabular}{llc}
% \toprule
% \textbf{Category}                                                                & \textbf{Corruption}        & \textbf{Modality} \\
% \midrule
%   \cellcolor{lightgray}& \cellcolor{lightgray}Rain (RN)                   & \cellcolor{lightgray}C, L             \\
%                                                                                  \cellcolor{lightgray}& \cellcolor{lightgray}Fog (FG)                    & \cellcolor{lightgray}C, L             \\
%                                                                                  \cellcolor{lightgray}& \cellcolor{lightgray}Brightness (BR)             & \cellcolor{lightgray}C              \\
%                                                                                  \cellcolor{lightgray}\multirow{-4}{*}{\begin{tabular}[l]{@{}l@{}}Weather  \\ Corruption\end{tabular}} & \cellcolor{lightgray}Darkness (DK)               & \cellcolor{lightgray}C              \\
% & Distortion (DT)            & C              \\
%                                                                                  & Motion blur (MB)            & C              \\
%                                                                                  \multirow{-3}{*}{\begin{tabular}[l]{@{}l@{}}Sensor \\ Corruption\end{tabular}}    & Defocus Blur (DB)          & C              \\
%       \cellcolor{lightgray}& \cellcolor{lightgray}Image Gaussion Noise (GN)        & \cellcolor{lightgray}C            \\
%       \cellcolor{lightgray}& \cellcolor{lightgray}Point Cloud Gaussion Noise (GN)        & \cellcolor{lightgray}L           \\
%       \cellcolor{lightgray}& \cellcolor{lightgray}Image Impulse  Noise (IN)        & \cellcolor{lightgray}C           \\
%                                                                                  \cellcolor{lightgray}\multirow{-4}{*}{\begin{tabular}[l]{@{}l@{}}Noise\\ Corruption\end{tabular}} & \cellcolor{lightgray}Point Cloud Impulse Noise (IN)         & \cellcolor{lightgray}L           \\
% &Spatial  misalignment (SM) &A              \\
%                                                                                  \multirow{-2}{*}{\begin{tabular}[l]{@{}l@{}}Sensor \\ Misalignment\end{tabular}} &Temporal misalignment (TM) &A             \\
% \bottomrule
% \end{tabular}
% \vspace{-10pt}
% \end{table}






% \newcommand{\tabBenchCorruption}[0]{
% \begin{table*}[]
% \caption{Common corruption patterns}
% \begin{tabular}{cllll}
% \textbf{CateGory}                                                               & \textbf{Corruption}   & \textbf{Sensor} & \textbf{Description}                & \textbf{Abbr} \\
% \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Weather  \\ Corruption\end{tabular}} & Rain                  & CL              & Weather conditions changes          & RN            \\
%                                                                                 & Fog                   & CL              & Weather conditions changes          & FG            \\
%                                                                                 & Bright                & C               & Lighting  conditions changes        & BR            \\
%                                                                                 & Dark                  & C               & Lighting  conditions changes        & DK            \\
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Sensor \\ Corruption\end{tabular}}   & Distortion            & C               & Optical lens inherent perspective distortion   & DT            \\
%                                                                                 & Motion Blur           & C               & Camera moves quickly                & MB            \\
%                                                                                 & Defocus Blur          & C               & Camera loses focus                  & DB            \\
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Noise \\ Corruption\end{tabular}}   & Gaussian Noise        & C,L             & Signal transmission noise           & GN            \\
%                                                                                 & Impulse Noise         & C,L             & Signal bit error                    & IN            \\
%                                                                                 & Loss                  & C,L             & Signal transmission failure         & LS            \\
% \multirow{2}{*}{Sensing \\ Misalignment}                                                & Spatial Misalignment  & A               & Timestamp synchronization failure   & SM            \\
%                                                                                 & Temporal Misalignment & A               & Recording error or sensor vibration & TM           
% \end{tabular}
% \end{table*}
% \label{tab: corruption}
% }



==> tab/benchMSF.tex <==
% \begin{table}[t]
% \scriptsize
% \centering
% \caption{The collected MSF systems (C and L represent \textit{camera} and \textit{LiDAR}).}
% \label{tab: fusion systems}
% \begin{tabular}{lcccc}
% \toprule
% \textbf{System}                    & \textbf{Task}    & \textbf{Fusion} & \textbf{Year} & \textbf{Modality} \\
% \midrule
% EPNet\cite{huang2020epnet}        & Object Detection & Deep            & 2020          & C+L            \\
% FConv\cite{wang2019frustum}       & Object Detection & Weak            & 2019          & C+L            \\
% CLOCs\cite{pang2020clocs}         & Object Detection & Late            & 2020          & C+L            \\
% JMODT\cite{huang2021jmodt}        & Object Tracking  & Deep            & 2021          & C+L            \\
% DFMOT\cite{wang2022deepfusionmot} & Object Tracking  & Late            & 2022          & C+L            \\
% TWISE\cite{imran2021twise}        & Depth Completion & Deep            & 2021          & C+L            \\
% MDANet\cite{ke2021mdanet}         & Depth Completion & Deep            & 2021          & C+L           
% \\\bottomrule
% \end{tabular}
% \vspace{-10pt}
% \end{table}

\begin{table}[t]
\scriptsize
\centering
\caption{The collected MSF systems. Performance of each system is evaluated by task-specific metrics (detailed in Sec.~\ref{sec: eval metrics}).}
\vspace{-10pt}
\label{tab: fusion systems}
 \resizebox{0.95\linewidth}{!}{%
\begin{tabular}{lccccc}
\toprule
\textbf{System}                    & \textbf{Task}    & \textbf{Fusion} & \textbf{Year} & \textbf{Modality} & \textbf{Performance} \\
\midrule
EPNet~\cite{huang2020epnet}        & Object Detection & Deep            & 2020          & C+L             & 82.70                \\
FConv~\cite{wang2019frustum}       & Object Detection & Weak            & 2019          & C+L             & 79.06                \\
CLOCs~\cite{pang2020clocs}         & Object Detection & Late            & 2020          & C+L             & 79.70                \\
JMODT~\cite{huang2021jmodt}        & Object Tracking  & Deep            & 2021          & C+L             & 86.12                \\
DFMOT~\cite{wang2022deepfusionmot} & Object Tracking  & Late            & 2022          & C+L             & 80.17                \\
TWISE~\cite{imran2021twise}        & Depth Completion & Deep            & 2021          & C+L             & 1009.64              \\
MDANet~\cite{ke2021mdanet}         & Depth Completion & Deep            & 2021          & C+L             & 898.39              
\\\bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{table}

==> tab/rq1rob.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \newcommand{\tabRqOneRob}[0]{
\begin{table*}[t]
\scriptsize
\caption{Average robustness performance of MSF systems against different corruption patterns across three severity levels.}
\vspace{-10pt}
\label{tab: rq1_rob}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{cc|cccc|ccc|cccc|cccc}
\toprule
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Task}}}   & \multicolumn{4}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Weather\end{tabular}}} & \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Sensor \end{tabular}}} & \multicolumn{4}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Noise\end{tabular}}} & \multirow{2}{*}{\textbf{$Rb^{s1}$}} & \multirow{2}{*}{\textbf{$Rb^{s2}$}} & \multirow{2}{*}{\textbf{$Rb^{s3}$}} & \multirow{2}{*}{\textbf{mRb}} \\

\multicolumn{2}{c|}{}                                 & RN                   & FG                   & BR                   & DK                   & DT                           & MB                           & DB                          & GN(C)                & GN(L)                & IN(C)               & IN(L)               &                               &                               &                               &                              \\
\midrule
\multirow{3}{*}{\textbf{Object}}   & \textbf{EPNet}  & 0.71                 & 0.35                 & 0.92                 & 0.83                 & 0.98                         & 0.90                         & 0.88                        & 0.98                 & 0.71                 & 0.98                & 0.79                & 0.90                          & 0.84                          & 0.72                          & 0.82                         \\
                                   & \textbf{FConv}  & 0.81                 & 0.43                 & 0.96                 & 0.84                 & 0.96                         & 0.66                         & 0.73                        & 0.66                 & 0.92                 & 0.66                & 0.92                & 0.93                          & 0.82                          & 0.58                          & 0.78                         \\
                                   & \textbf{CLOCs}  & 0.69                 & 0.41                 & 0.97                 & 0.85                 & 0.99                         & 0.70                         & 0.76                        & 0.67                 & 0.85                 & 0.68                & 0.95                & 0.92                          & 0.83                          & 0.58                          & 0.77                         \\

\midrule
\multirow{2}{*}{\textbf{Tracking}} & \textbf{JMODT}  & 0.79                 & 0.26                 & 0.92                 & 0.75                 & 0.97                         & 0.88                         & 0.81                        & 0.86                 & 0.81                 & 0.86                & 0.94                & 0.89                          & 0.82                          & 0.70                          & 0.80                         \\
                                   & \textbf{DFMOT}  & 0.84                 & 0.41                 & 0.95                 & 0.77                 & 0.98                         & 0.54                         & 0.57                        & 0.59                 & 0.95                 & 0.60                & 0.99                & 0.92                          & 0.78                          & 0.54                          & 0.75                         \\
\midrule
\multirow{2}{*}{\textbf{Depth}}    & \textbf{TWISE}  & 0.56                 & 0.05                 & 0.99                 & 0.88                 & 0.94                         & 0.94                         & 0.93                        & 0.95                 & 0.95                 & 0.95                & 0.98                & 0.87                          & 0.83                          & 0.79                          & 0.83                         \\
                                   & \textbf{MDANet} & 0.62                 & 0.14                 & 0.99                 & 0.86                 & 0.92                         & 0.92                         & 0.90                        & 0.49                 & 0.96                 & 0.46                & 0.98                & 0.89                          & 0.72                          & 0.64                          & 0.75                         \\
\midrule
\multicolumn{2}{c|}{\textbf{Avg}}                     & 0.72                 & 0.29                 & 0.96                 & 0.83                 & 0.96                         & 0.79                         & 0.80                        & 0.74                 & 0.88                 & 0.74                & 0.94                & 0.90                          & 0.81                          & 0.65                          & 0.67                        
\\\bottomrule
\end{tabular}
}
\vspace{-5pt}
\end{table*}
% }




==> tab/rq1rob2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \newcommand{\tabRqOneRob}[0]{
\begin{table*}[t]
\scriptsize
\caption{Performance of MSF systems against different corruption patterns.}
\label{tab: rq1_rob}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cc|cccc|ccc|cccc|cccc}
\toprule
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Task}}}   & \multicolumn{4}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Weather\end{tabular}}} & \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Sensor \end{tabular}}} & \multicolumn{4}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Noise\end{tabular}}} & \multirow{2}{*}{\textbf{$Rb^{s1}$}} & \multirow{2}{*}{\textbf{$Rb^{s2}$}} & \multirow{2}{*}{\textbf{$Rb^{s3}$}} & \multirow{2}{*}{\textbf{mRb}} \\

\multicolumn{2}{c|}{}                                 & RN                   & FG                   & BR                   & DK                   & DT                           & MB                           & DB                          & GN(C)                & GN(L)                & IN(C)               & IN(L)               &                               &                               &                               &                              \\
\midrule
\multirow{3}{*}{\textbf{Object}}   & \textbf{EPNet}  & 70.6                 & 35.0                 & 91.8                 & 83.1                 & 98.3                         & 90.1                         & 87.9                        & 97.5                 & 71.1                 & 97.9                & 79.4                & 89.8                          & 84.1                          & 72.2                          & 82.1                         \\
                                   & \textbf{FConv}  & 81.0                 & 43.3                 & 95.6                 & 84.1                 & 95.9                         & 65.6                         & 73.3                        & 66.1                 & 91.7                 & 66.3                & 91.7                & 93.5                          & 82.0                          & 57.6                          & 77.7                         \\
                                   & \textbf{CLOCs}  & 68.9                 & 40.7                 & 96.8                 & 85.3                 & 99.0                         & 70.1                         & 76.2                        & 67.2                 & 85.2                 & 68.0                & 95.0                & 91.9                          & 82.8                          & 57.8                          & 77.5                         \\
\midrule
\multirow{2}{*}{\textbf{Tracking}} & \textbf{JMODT}  & 78.9                 & 25.9                 & 92.2                 & 74.8                 & 96.7                         & 88.0                         & 81.0                        & 86.2                 & 80.7                 & 86.0                & 93.7                & 89.4                          & 82.0                          & 62.2                          & 80.4                         \\
                                   & \textbf{DFMOT}  & 84.2                 & 40.7                 & 94.9                 & 76.5                 & 98.0                         & 54.4                         & 57.3                        & 59.3                 & 95.1                 & 60.0                & 99.0                & 91.5                          & 78.1                          & 53.9                          & 74.5                         \\
\midrule
\multirow{2}{*}{\textbf{Depth}}    & \textbf{TWISE}  & 56.2                 & 4.7                  & 99.3                 & 87.8                 & 94.1                         & 94.4                         & 93.2                        & 95.3                 & 95.3                 & 95.5                & 98.0                & 87.2                          & 82.6                          & 79.5                          & 83.1                         \\
                                   & \textbf{MDANet} & 62.5                 & 14.0                 & 99.2                 & 86.4                 & 91.9                         & 91.7                         & 90.4                        & 49.1                 & 96.2                 & 45.5                & 98.0                & 88.9                          & 72.0                          & 64.1                          & 75.0                         \\
\midrule
\multicolumn{2}{c|}{\textbf{Avg}}                     & 71.8                 & 29.2                 & 95.7                 & 82.6                 & 96.3                         & 79.2                         & 79.9                        & 74.4                 & 87.9                 & 74.2                & 89.6                & 90.3                          & 80.5                          & 63.9                          & 78.2                        
\\\bottomrule
\end{tabular}
}
\end{table*}
% }




==> tab/rq2loss.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \newcommand{\tabRqTwoLoss}[0]{
\begin{table}[tb]
\small
\caption{MSF systems' performance when completely losing one source of the signals.}
\vspace{-10pt}
\label{tab: rq2_loss}
\resizebox{0.95\linewidth}{!}{%
\setlength{\tabcolsep}{0.9mm}{
\begin{tabular}{cccccccc}
\toprule
\textbf{Modality} & \multicolumn{1}{l}{\textbf{EPNet}} & \multicolumn{1}{l}{\textbf{FConv}} & \multicolumn{1}{l}{\textbf{CLOCs}} & \multicolumn{1}{l}{\textbf{JMODT}} & \multicolumn{1}{l}{\textbf{DFMOT}} & \multicolumn{1}{l}{\textbf{TWISE}} & \multicolumn{1}{l}{\textbf{MDANet}} \\
\midrule
C                 & 0.23                               & 0                                  & 0                                  & 0.13                               & 0                                  & 0.50                               & 0.58                                \\
L                 & 0                                  & 0                                  & 0                                  & 0                                  & 0                                  & 0                                  & 0   
\\\bottomrule
\end{tabular}
}
}
\vspace{-10pt}
\end{table}
% }



==> tab/rq3_calib.tex <==
\begin{table}[t]

\scriptsize
 % \caption{Spatial misalignment of different aixs.}
 \caption{Robustness performance of MSF systems against spatial misalignment.}
 \vspace{-10pt}
 \label{tab: rq3_sp_mis}
 \resizebox{0.9\linewidth}{!}{%
\setlength{\tabcolsep}{0.8mm}{
\begin{tabular}{cc|ccccccc}
\toprule
\multicolumn{2}{c|}{\textbf{Axis}} & \textbf{EPNet} & \textbf{FConv} & \textbf{CLOCs} & \textbf{JMODT} & \textbf{DFMOT} & \textbf{TWISE} & \textbf{MDANet} \\
\midrule
\multirow{3}{*}{X}                           & 0.5°                           & 0.93           & 0.92           & 0.96           & 0.98           & 0.99           & 0.94           & 0.94            \\
                                             & 1°                             & 0.80           & 0.79           & 0.83           & 0.94           & 0.99           & 0.82           & 0.83            \\
                                             & 2°                             & 0.46           & 0.48           & 0.57           & 0.80           & 0.72           & 0.57           & 0.58            \\
\midrule
\multirow{3}{*}{Y}                   & 0.5°                                   & 0.45                 & 0.41                 & 0.41                    & 0.93                 & 0.84                 & 0.73                 & 0.77                 \\
                                     & 1°                                     & 0.09                 & 0.04                 & 0.04                    & 0.54                 & 0.75                 & 0.16                 & 0.34                 \\
                                     & \cellcolor{tab_red}2°                  & \cellcolor{tab_red}0 & \cellcolor{tab_red}0 & \cellcolor{tab_red}0.06 & \cellcolor{tab_red}0 & \cellcolor{tab_red}0 & \cellcolor{tab_red}0 & \cellcolor{tab_red}0 \\
\midrule                                       
\multirow{3}{*}{Z}                      & 0.5°                                & 0.93           & 0.92           & 0.96             & 0.98           & 0.99           & 0.94           & 0.94            \\
                                        & 1°                                  & 0.80           & 0.79           & 0.83             & 0.95           & 0.99           & 0.82           & 0.83            \\
                                        & 2°                                  & 0.44           & 0.48           & 0.56             & 0.80           & 0.72           & 0.57           & 0.59            \\
\midrule
\multicolumn{2}{c|}{Avg}                                                       & 0.54                 & 0.54                 & 0.58                    & 0.77                 & 0.77                 & 0.62                 & 0.65                


\\\bottomrule
\end{tabular}
}
}
\vspace{-5pt}
\end{table}
% }

==> tab/rq3_calib2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \newcommand{\tabRqThreeCalib}[0]{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]

\scriptsize
 % \caption{Spatial misalignment of different aixs.}
 \caption{Robustness performance of MSF systems against spatial misalignment.}
 \label{tab: rq3_sp_mis}
 \resizebox{\linewidth}{!}{%
\setlength{\tabcolsep}{0.8mm}{
\begin{tabular}{cc|ccccccc}
\toprule
\multicolumn{2}{c|}{\textbf{Axis}} & \textbf{EPNet} & \textbf{FConv} & \textbf{CLOCs} & \textbf{JMODT} & \textbf{DFMOT} & \textbf{TWISE} & \textbf{MDANet} \\
\midrule
\multirow{3}{*}{X}     & 0.5°     & 92.7           & 92.1           & 96.1           & 97.9           & 99.5           & 93.7           & 94.2            \\
                       & 1°       & 79.6           & 79             & 83.2           & 94.3           & 99.6           & 82.1           & 83.1            \\
                       & 2°       & 46.2           & 48             & 56.5           & 80.3           & 71.5           & 56.8           & 58.4            \\
\midrule
\multirow{3}{*}{Y}                   & 0.5°                                   & 0.45                 & 0.41                 & 0.41                    & 0.93                 & 0.84                 & 0.73                 & 0.77                 \\
                                     & 1°                                     & 0.09                 & 0.04                 & 0.04                    & 0.54                 & 0.75                 & 0.16                 & 0.34                 \\
                                     & \cellcolor{tab_red}2°                  & \cellcolor{tab_red}0 & \cellcolor{tab_red}0 & \cellcolor{tab_red}0.06 & \cellcolor{tab_red}0 & \cellcolor{tab_red}0 & \cellcolor{tab_red}0 & \cellcolor{tab_red}0 \\
\midrule
\multirow{3}{*}{Z}     & 0.5°     & 92.7           & 91.9           & 96.3           & 98             & 99.6           & 93.8           & 94.3            \\
                       & 1°       & 79.7           & 79.4           & 83.3           & 95.1           & 98.6           & 82.3           & 83.3            \\
                       & 2°       & 44.1           & 48.1           & 55.8           & 80             & 71.5           & 57             & 58.8           
\\\midrule
\multicolumn{2}{c|}{Avg}                                                       & 54.31          & 53.76          & 58.02          & 76.88          & 77.66          & 61.63          & 64.72

\\\bottomrule
\end{tabular}
}
}
\end{table}
% }

==> tab/rq4_sigloss.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
 \caption{
Improved performance of CLOCs-Rb and FConv-Rb against partial or complete signal loss.}
\vspace{-10pt}
 \label{tab: rq4_sig_mis}
 \resizebox{0.95\linewidth}{!}{%
\begin{tabular}{cccccccc}
\toprule
\multicolumn{1}{l}{\textbf{Systems}} & \textbf{Modality} & 10\%    & 25\%    & 50\%   & 75\%    & 100\%  & Avg  \\
\midrule
\multirow{2}{*}{\textbf{CLOCs-Rb}}   & C                 & -0.01 & 0.07  & 0.41 & 0.86  & \cellcolor{tab_red}0.94 & 0.45 \\
                                     & L                 & -0.01 & -0.01 & 0.00 & -0.01 & 0    & 0.00 \\

\multirow{2}{*}{\textbf{FConv-Rb}}   & C                 & 0.00  & 0.10  & 0.52 & 0.86  & \cellcolor{tab_red}0.99 & 0.49 \\
                                     & L                 & 0.00  & 0.00  & 0.00 & 0.00  & 0    & 0.00
\\
\bottomrule
\end{tabular}
}
\vspace{-15pt}
\end{table}

==> tab/sim_weather.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table}[t]
\caption{Classification accuracy on validation and test data.}
\label{tab: sim_weather_acc}
 \resizebox{0.95\linewidth}{!}{
\begin{tabular}{ccccc}
\toprule
\textbf{Corruption} & \textbf{Dataset} & \textbf{Size} & \textbf{Val Accuracy} & \textbf{Test Accuracy} \\
\midrule
Fog        & Dense\cite{bijelic2020seeing}   & 1200 &  97.2\%     &       98.6\%  \\
Rain       & Boreas\cite{burnett2022boreas}  & 1144 &  98.3\%       &     98.0\%  \\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{table}

